WARM-3D: A Weakly-Supervised Sim2Real Domain Adaptation Framework for Roadside Monocular 3D Object Detection

Existing roadside perception systems are limited by the absence of publicly available, large-scale, high-quality 3D datasets. Exploring the use of cost-effective, extensive synthetic datasets offers a viable solution to tackle this challenge and enhance the performance of roadside monocular 3D detection. In this study, we introduce the TUMTraf Synthetic Dataset, offering a diverse and substantial collection of high-quality 3D data to augment scarce real-world datasets. Besides, we present WARM-3D, a concise yet effective framework to aid the Sim2Real domain transfer for roadside monocular 3D detection. Our method leverages cheap synthetic datasets and 2D labels from an off-the-shelf 2D detector for weak supervision. We show that WARM-3D significantly enhances performance, achieving a +12.40% increase in mAP 3D over the baseline with only pseudo-2D supervision. With 2D GT as weak labels, WARM-3D even reaches performance close to the Oracle baseline. Moreover, WARM-3D improves the ability of 3D detectors to unseen sample recognition across various real-world environments, highlighting its potential for practical applications.

==> table/ablation_dynamics.tex <==

%  metrics can change to categories level
\begin{table}[htb!]
\centering
\footnotesize 
\caption{Evaluation result of using different thresholds of Confidence-aware bipartite matching on TUM-Traf-I Image Dataset.} 
\resizebox{0.48\textwidth}{!}{
% \begin{tabular}{cccccccccc}
% \toprule[0.5pt]
% \multirow{2}{*}{\textbf{Threshold}}& \multirow{2}{*}{\textbf{Precision}} & \multirow{2}{*}{\textbf{Recall}} & \multicolumn{4}{c}{$\textbf{mAP}_{\textbf{3D}}$} \\
% & & ~ & Easy & Mod. & Hard & Overall \\ 
% \midrule[0.5pt]

% 0.1 & 38.16 & 38.87 & 51.61 & 30.73 & 22.40 & 37.45 \\

% 1.0 & 35.20 & 38.57 & 49.53 & \textbf{34.96} & 20.28 & 34.53 \\

% 2.0 & 38.97 & 38.48 & \textbf{54.18} & 33.73 & \textbf{23.06} & \textbf{39.17} \\

% 2.5 & 36.57 & 37.66 & 54.04 & 28.72 & 18.07 & 35.91 \\

% % ... add more

% \bottomrule[0.5pt]
    
% \end{tabular}
        \begin{tabular}{cccccccccc}
            \toprule[0.5pt]
            \multirow{2}{*}{\textbf{Threshold}} & \multirow{2}{*}{\textbf{Precision}} & \multirow{2}{*}{\textbf{Recall}} & \multicolumn{4}{c}{$\textbf{mAP}_{\textbf{3D}}$}                                                    \\
                                                &                                     & ~                                & Easy                                             & Mod.           & Hard           & Overall        \\
            \midrule[0.5pt]

            0.2                                 & 35.47                               & 35.86                            & 49.42                                            & 27.85          & 19.90          & 34.80          \\

            1.0                                 & 38.46                               & 38.42                            & 52.00                                            & 31.66          & 22.37          & 37.74          \\

            2.0                                 & 37.74                               & 36.60                            & 51.50                                            & 35.08          & 20.39          & 37.12          \\

            2.2                                 & \textbf{42.23}                      & \textbf{39.84 }                  & \textbf{55.09}                                   & 35.17          & \textbf{24.89} & \textbf{41.55} \\

            2.8                                 & 40.67                               & 39.00                            & 51.88                                            & \textbf{38.70} & 23.26          & 39.95          \\

            % ... add more

            \bottomrule[0.5pt]
        \end{tabular}
}

\label{tab:Ablation-dynamics}
\vspace{-1em}

\end{table}


